Are You Satisfied by This Partial Assignment?

Many procedures for SAT and SAT-related problems -- in particular for those requiring the complete enumeration of satisfying truth assignments -- rely their efficiency on the detection of partial assignments satisfying an input formula. In this paper we analyze the notion of partial-assignment satisfiability -- in particular when dealing with non-CNF and existentially-quantified formulas -- raising a flag about the ambiguities and subtleties of this concept, and investigating their practical consequences. This may drive the development of more effective assignment-enumeration algorithms.

==> TAGS <==

background.tex,626
The symbols $\alla\defas\set{as\set39,1268
$\allb\defas\set{as\set40,1315
Given $\alla\defas\set{as\set97,3305
We assume $\eta(\top)\defas \trueval$ and $\eta(\bot)\defas \falseval$.as101,3450
$\eta\defas \set{as104,3572
$\alla'\subseteq A$ and $N'\defas||\alla'||$.as||\alla'||$.116,4094
\label{prop:total-properties}prop:total-properties197,7188
{Notice that Property~\ref{prop:total-properties}prop:total-properties214,7674
CNF-ization \cite{tseitin1}tseitin1223,8083
$CNF(B \iff (l_1 \wedge l_2)) \defas as233,8528
\shannonpsib\defas as257,9490
\label{prop:total-shannon}prop:total-shannon267,9764

figure.tex,331
\newcommand{\mainwff}\mainwff1,0
\newcommand{\wffl}\wffl2,77
\newcommand{\wffr}\wffr3,127
\newcommand{\Aone}\Aone4,181
\newcommand{\nAone}\nAone5,218
\newcommand{\Atwo}\Atwo6,261
\newcommand{\nAtwo}\nAtwo7,298
\caption{Left: OBDD for $\vi\defas\mainwff{as\mainwff12,422
\label{fig:comparison}fig:comparison15,572

intro.tex,668
\cite{bryant2}bryant27,233
\cite{davis7}davis78,290
\cite{GSS09HBSAT}GSS09HBSAT14,540
\cite{allsmt}allsmt15,606
\cite{ST09HBSAT}ST09HBSAT16,668
formulas (e.g.  \cite{KBK09HBSAT}KBK09HBSAT27,1240
formulas (e.g. \cite{KBK09HBSAT}KBK09HBSAT84,3492
OBDDs \cite{bryant2}bryant2109,4362
the input formulas, whereas Analytic Tableaux \cite{smullyan1}smullyan1110,4439
(non-CNF) DPLL \cite{davis7}davis7111,4506
\cite{sebastiani07,BSST09HBSAT}sebastiani07,BSST09HBSAT117,4693
The result are available at \cite{poll}poll145,5861
\cite{MorPasSeb17,morettin_aij19}MorPasSeb17,morettin_aij19162,6551
 (see \cite{gs-infocomp2000}gs-infocomp2000166,6757

jsat_main.tex,1091
\renewcommand{\topfraction}\topfraction19,393
\renewcommand{\bottomfraction}\bottomfraction20,424
\renewcommand{\textfraction}\textfraction21,458
\newcommand{\longversion}\longversion86,2095
  \renewcommand{\ignoreinshort}\ignoreinshort90,2173
  \renewcommand{\ignoreinshort}\ignoreinshort91,2230
  \renewcommand{\ignoreinlong}\ignoreinlong92,2271
 \renewcommand{\ignoreinshort}\ignoreinshort95,2313
 \renewcommand{\ignoreinlong}\ignoreinlong96,2349
\section{Motivations and Goals}Motivations152,3278
\label{sec:intro}sec:intro153,3310
\section{Background}Background160,3482
\label{sec:background}sec:background161,3503
\section{Partial-assignment satisfiability for propositional formulas}Partial-assignment165,3556
\label{sec:partialsat}sec:partialsat166,3627
\section{Dealing with existentially-quantified formulas}Dealing170,3680
\label{sec:partialsat-exist}sec:partialsat-exist171,3737
\section{A simple poll}A175,3801
\label{sec:poll}sec:poll176,3825
\section{Conclusions and Future Work}Conclusions179,3857
\label{sec:concl}sec:concl180,3895

main.tex,1087
\renewcommand{\topfraction}\topfraction5,79
\renewcommand{\bottomfraction}\bottomfraction6,110
\renewcommand{\textfraction}\textfraction7,144
\newcommand{\longversion}\longversion63,1529
  \renewcommand{\ignoreinshort}\ignoreinshort67,1607
  \renewcommand{\ignoreinshort}\ignoreinshort68,1664
  \renewcommand{\ignoreinlong}\ignoreinlong69,1705
 \renewcommand{\ignoreinshort}\ignoreinshort72,1747
 \renewcommand{\ignoreinlong}\ignoreinlong73,1783
\section{Motivations and Goals}Motivations128,2619
\label{sec:intro}sec:intro129,2651
\section{Background}Background136,2823
\label{sec:background}sec:background137,2844
\section{Partial-assignment satisfiability for propositional formulas}Partial-assignment141,2897
\label{sec:partialsat}sec:partialsat142,2968
\section{Dealing with existentially-quantified formulas}Dealing146,3021
\label{sec:partialsat-exist}sec:partialsat-exist147,3078
\section{A simple poll}A151,3142
\label{sec:poll}sec:poll152,3166
\section{Conclusions and Future Work}Conclusions155,3198
\label{sec:concl}sec:concl156,3236

partialsat-exist.tex,1789
(see e.g. \cite{burch1}burch13,117
(see e.g. \cite{graf_predabs97,beyercgks09}graf_predabs97,beyercgks094,192
{\em entailment}, leveraging Definition~\ref{def:entailment}def:entailment18,784
and Property~\ref{prop:total-shannon}prop:total-shannon19,845
that is, by Property~\ref{prop:total-shannon}prop:total-shannon22,1054
\label{def:entailment-exist}def:entailment-exist29,1324
\label{remark:nestingorder}remark:nestingorder51,2035
Definition~\ref{def:entailment-exist}def:entailment-exist53,2128
{\em validation}, leveraging Definition~\ref{def:validation}def:validation73,2980
and Property~\ref{prop:total-shannon}prop:total-shannon74,3041
\label{def:validation-exist}def:validation-exist83,3470
Due to Proposition~\ref{prop:stronger}prop:stronger104,4091
Property~\ref{prop:total-shannon}prop:total-shannon105,4134
 (Definition~\ref{def:validation-exist}def:validation-exist107,4215
 (Definition~\ref{def:entailment-exist}def:entailment-exist109,4314
\begin{example} Consider $\mu\defas\set{as\set117,4618
\psi\defas  as121,4745
\subsection{A Relevant Example Application: Predicate Abstraction.}A152,5574
  \label{eq:predabs}eq:predabs166,6122
 \predabsphi \defasas167,6143
\cite{graf_predabs97,allsmt,cavada_fmcad07_predabs}graf_predabs97,allsmt,cavada_fmcad07_predabs176,6386
  \cite{graf_predabs97,allsmt,cavada_fmcad07_predabs}graf_predabs97,allsmt,cavada_fmcad07_predabs181,6720
$\phi\defas(\neg B_1\vee B_2)\wedge (B_1\vee \neg B_2)$as(\neg197,7436
$\Phi_1\defas B_1\wedge B_2$ andas199,7527
$\Phi_2\defas \neg B_1\wedge B_2$.as200,7560
  \label{eq:predabs1}eq:predabs1203,7617
  \predabsphi &\defas & \exists B_1 B_2. \left (as204,7639
  \label{eq:predabs2}eq:predabs2212,7865
  \label{eq:predabs3}eq:predabs3215,7953

partialsat.tex,3169
\label{def:entailment}def:entailment10,348
\label{def:validation}def:validation23,742
In substance, Definition~\ref{def:entailment}def:entailment32,997
assignments Property~\ref{prop:total-properties}prop:total-properties33,1062
Definition~\ref{def:validation}def:validation34,1124
Property~\ref{prop:total-properties}prop:total-properties36,1188
should verify all statements in Property~\ref{prop:total-properties}prop:total-properties39,1301
then Definitions~\ref{def:entailment}def:entailment47,1630
\ref{def:validation}def:validation48,1672
we notice that Definitions~\ref{def:entailment}def:entailment63,2273
\ref{def:validation}def:validation64,2325
if $\vi\defas(A_1\wedge A_2)\vee (A_1\wedge \neg A_2)$ and as(A_1\wedge71,2636
$\mu\defas\set{as\set72,2696
\label{prop:stronger}prop:stronger79,2832
$\mu\defas\set{as\set91,3131
$\vi\defas\bigvee_i (A_i\wedge cube_i)$ s.t. each $cube_i$ is a cube and $\bigvee_i cube_i$ isas\bigvee_i92,3174
We try to build a counterpart of Property~\ref{prop:total-properties}prop:total-properties99,3486
for Definitions~\ref{def:entailment}def:entailment100,3556
\ref{def:validation}def:validation101,3597
achieve all points (i)-(iv) in Property~\ref{prop:total-properties}prop:total-properties102,3661
From Definition~\ref{def:entailment}def:entailment108,3933
\label{prop:partial-entailment}prop:partial-entailment112,4014
Property~\ref{prop:total-properties}prop:total-properties133,4687
even partial ones (Property~\ref{prop:partial-entailment}prop:partial-entailment141,5038
is co-NP-complete  (Property~\ref{prop:partial-entailment}prop:partial-entailment144,5172
From Definition~\ref{def:validation}def:validation170,5848
\label{prop:partial-validation}prop:partial-validation174,5929
and practical need that the process of checking it should be fast (Property~\ref{prop:partial-validation}prop:partial-validation194,6653
assignments  (Property~\ref{prop:partial-validation}prop:partial-validation200,6921
Due to Proposition~\ref{prop:stronger}prop:stronger205,7090
OBDDs \cite{bryant2}bryant2218,7519
(Definition~\ref{def:entailment}def:entailment220,7627
valid (Property~\ref{prop:partial-entailment}prop:partial-entailment222,7709
 or subsumed  assignments (see \cite{dagostino1,gs-infocomp2000}dagostino1,gs-infocomp2000227,7957
\cite{smullyan1}smullyan1228,8024
\footnote{Classic DPLL procedure \cite{davis7}davis7230,8070
procedure (see e.g. \cite{armando5}armando5233,8223
\cite{davis7}davis7235,8265
(Definition~\ref{def:validation}def:validation237,8368
Figure~\ref{fig:comparison}fig:comparison250,8835
represents the OBDD for $\vi\defas\mainwff$ and as\mainwff$251,8864
\footnote{Here in DPLL the pure-literal rule \cite{davis7}davis7256,9019
 some relevant models (see, e.g., \cite{sebastiani_frocos07}sebastiani_frocos07258,9144
Consider $\vi\defas A_1 \vee (A_2\wedge A_3)$ as290,10587
\psi\defas & (A_1\vee  B_1)\ \wedge \\as294,10691
On the one hand, $\mu\defas \set{as300,10879
Consider $\vi\defasas305,11153
\psi\defas  as311,11279
Although $\mu\defas \set{as330,11873
\cite{tseitin1}tseitin1349,12675

poll.tex,1302
\renewcommand{\topfraction}\topfraction6,108
\renewcommand{\bottomfraction}\bottomfraction7,139
\renewcommand{\textfraction}\textfraction8,173
\newcommand{\longversion}\longversion65,1559
  \renewcommand{\ignoreinshort}\ignoreinshort69,1637
  \renewcommand{\ignoreinshort}\ignoreinshort70,1694
  \renewcommand{\ignoreinlong}\ignoreinlong71,1735
 \renewcommand{\ignoreinshort}\ignoreinshort74,1777
 \renewcommand{\ignoreinlong}\ignoreinlong75,1813
\label{sec:}sec:134,2706
\section*{*145,3121
\section*{*157,3541
\section*{*223,5260
$\alla\defas\set{as\set227,5327
$\allb\defas\set{as\set228,5359
\section*{*258,6404
Here follow the complete results (table \ref{tab:results}tab:results259,6423
of answers (table \ref{tab:results_summary}tab:results_summary261,6560
  \label{tab:results}tab:results330,8857
  \label{tab:results_summary}tab:results_summary331,8879
\section*{*335,8923
topic  \cite{sat19}sat19339,9024
Property 3(ii), Remark 1, and Definition 4 in \cite{sat19}sat19344,9202
  satisfiability as entailment (Definition 1 in \cite{sat19}sat19348,9333
  satisfiability as validation (Definition 2 in \cite{sat19}sat19350,9451
\item According to Proposition 1 in \cite{sat19}sat19351,9515
  Properties 5 and 6 in \cite{sat19}sat19364,10202

rgb.tex,16818
\definecolor {inecolor18,747
\definecolor {inecolor19,804
\definecolor {inecolor20,861
\definecolor {inecolor21,918
\definecolor {inecolor22,975
\definecolor {inecolor23,1032
\definecolor {inecolor24,1089
\definecolor {inecolor25,1146
\definecolor {inecolor26,1203
\definecolor {inecolor27,1260
\definecolor {inecolor28,1317
\definecolor {inecolor29,1374
\definecolor {inecolor30,1431
\definecolor {inecolor31,1488
\definecolor {inecolor32,1545
\definecolor {inecolor33,1602
\definecolor {inecolor34,1659
\definecolor {inecolor35,1716
\definecolor {inecolor36,1773
\definecolor {inecolor37,1830
\definecolor {inecolor38,1887
\definecolor {inecolor39,1944
\definecolor {inecolor40,2001
\definecolor {inecolor41,2058
\definecolor {inecolor42,2115
\definecolor {inecolor43,2172
\definecolor {inecolor44,2229
\definecolor {inecolor45,2286
\definecolor {inecolor46,2343
\definecolor {inecolor47,2400
\definecolor {inecolor48,2457
\definecolor {inecolor49,2514
\definecolor {inecolor50,2571
\definecolor {inecolor51,2628
\definecolor {inecolor52,2685
\definecolor {inecolor53,2742
\definecolor {inecolor54,2799
\definecolor {inecolor55,2856
\definecolor {inecolor56,2913
\definecolor {inecolor57,2970
\definecolor {inecolor58,3027
\definecolor {inecolor59,3084
\definecolor {inecolor60,3141
\definecolor {inecolor61,3198
\definecolor {inecolor62,3255
\definecolor {inecolor63,3312
\definecolor {inecolor64,3369
\definecolor {inecolor65,3426
\definecolor {inecolor66,3483
\definecolor {inecolor67,3540
\definecolor {inecolor68,3597
\definecolor {inecolor69,3654
\definecolor {inecolor70,3711
\definecolor {inecolor71,3768
\definecolor {inecolor72,3825
\definecolor {inecolor73,3882
\definecolor {inecolor74,3939
\definecolor {inecolor75,3996
\definecolor {inecolor76,4053
\definecolor {inecolor77,4110
\definecolor {inecolor78,4167
\definecolor {inecolor79,4224
\definecolor {inecolor80,4281
\definecolor {inecolor81,4338
\definecolor {inecolor82,4395
\definecolor {inecolor83,4452
\definecolor {inecolor84,4509
\definecolor {inecolor85,4566
\definecolor {inecolor86,4623
\definecolor {inecolor87,4680
\definecolor {inecolor88,4737
\definecolor {inecolor89,4794
\definecolor {inecolor90,4851
\definecolor {inecolor91,4908
\definecolor {inecolor92,4965
\definecolor {inecolor93,5022
\definecolor {inecolor94,5079
\definecolor {inecolor95,5136
\definecolor {inecolor96,5193
\definecolor {inecolor97,5250
\definecolor {inecolor98,5307
\definecolor {inecolor99,5365
\definecolor {inecolor100,5422
\definecolor {inecolor101,5479
\definecolor {inecolor102,5536
\definecolor {inecolor103,5593
\definecolor {inecolor104,5650
\definecolor {inecolor105,5707
\definecolor {inecolor106,5764
\definecolor {inecolor107,5821
\definecolor {inecolor108,5878
\definecolor {inecolor109,5935
\definecolor {inecolor110,5992
\definecolor {inecolor111,6049
\definecolor {inecolor112,6106
\definecolor {inecolor113,6163
\definecolor {inecolor114,6220
\definecolor {inecolor115,6277
\definecolor {inecolor116,6334
\definecolor {inecolor117,6391
\definecolor {inecolor118,6448
\definecolor {inecolor119,6505
\definecolor {inecolor120,6562
\definecolor {inecolor121,6619
\definecolor {inecolor122,6676
\definecolor {inecolor123,6733
\definecolor {inecolor124,6790
\definecolor {inecolor125,6847
\definecolor {inecolor126,6904
\definecolor {inecolor127,6961
\definecolor {inecolor128,7018
\definecolor {inecolor129,7075
\definecolor {inecolor130,7132
\definecolor {inecolor131,7189
\definecolor {inecolor132,7246
\definecolor {inecolor133,7303
\definecolor {inecolor134,7360
\definecolor {inecolor135,7417
\definecolor {inecolor136,7474
\definecolor {inecolor137,7531
\definecolor {inecolor138,7588
\definecolor {inecolor139,7645
\definecolor {inecolor140,7702
\definecolor {inecolor141,7759
\definecolor {inecolor142,7816
\definecolor {inecolor143,7873
\definecolor {inecolor144,7930
\definecolor {inecolor145,7987
\definecolor {inecolor146,8044
\definecolor {inecolor147,8101
\definecolor {inecolor148,8158
\definecolor {inecolor149,8215
\definecolor {inecolor150,8272
\definecolor {inecolor151,8329
\definecolor {inecolor152,8386
\definecolor {inecolor153,8443
\definecolor {inecolor154,8500
\definecolor {inecolor155,8557
\definecolor {inecolor156,8614
\definecolor {inecolor157,8671
\definecolor {inecolor158,8728
\definecolor {inecolor159,8785
\definecolor {inecolor160,8842
\definecolor {inecolor161,8899
\definecolor {inecolor162,8956
\definecolor {inecolor163,9013
\definecolor {inecolor164,9070
\definecolor {inecolor165,9127
\definecolor {inecolor166,9184
\definecolor {inecolor167,9241
\definecolor {inecolor168,9298
\definecolor {inecolor169,9355
\definecolor {inecolor170,9412
\definecolor {inecolor171,9469
\definecolor {inecolor172,9526
\definecolor {inecolor173,9583
\definecolor {inecolor174,9640
\definecolor {inecolor175,9697
\definecolor {inecolor176,9754
\definecolor {inecolor177,9811
\definecolor {inecolor178,9868
\definecolor {inecolor179,9925
\definecolor {inecolor180,9982
\definecolor {inecolor181,10039
\definecolor {inecolor182,10096
\definecolor {inecolor183,10153
\definecolor {inecolor184,10210
\definecolor {inecolor185,10267
\definecolor {inecolor186,10324
\definecolor {inecolor187,10381
\definecolor {inecolor188,10438
\definecolor {inecolor189,10495
\definecolor {inecolor190,10552
\definecolor {inecolor191,10609
\definecolor {inecolor192,10666
\definecolor {inecolor193,10723
\definecolor {inecolor194,10780
\definecolor {inecolor195,10837
\definecolor {inecolor196,10894
\definecolor {inecolor197,10951
\definecolor {inecolor198,11008
\definecolor {inecolor199,11065
\definecolor {inecolor200,11122
\definecolor {inecolor201,11179
\definecolor {inecolor202,11236
\definecolor {inecolor203,11293
\definecolor {inecolor204,11350
\definecolor {inecolor205,11407
\definecolor {inecolor206,11464
\definecolor {inecolor207,11521
\definecolor {inecolor208,11578
\definecolor {inecolor209,11635
\definecolor {inecolor210,11692
\definecolor {inecolor211,11749
\definecolor {inecolor212,11806
\definecolor {inecolor213,11863
\definecolor {inecolor214,11920
\definecolor {inecolor215,11977
\definecolor {inecolor216,12034
\definecolor {inecolor217,12091
\definecolor {inecolor218,12148
\definecolor {inecolor219,12205
\definecolor {inecolor220,12262
\definecolor {inecolor221,12319
\definecolor {inecolor222,12376
\definecolor {inecolor223,12433
\definecolor {inecolor224,12490
\definecolor {inecolor225,12547
\definecolor {inecolor226,12604
\definecolor {inecolor227,12661
\definecolor {inecolor228,12718
\definecolor {inecolor229,12775
\definecolor {inecolor230,12832
\definecolor {inecolor231,12889
\definecolor {inecolor232,12946
\definecolor {inecolor233,13003
\definecolor {inecolor234,13060
\definecolor {inecolor235,13117
\definecolor {inecolor236,13174
\definecolor {inecolor237,13231
\definecolor {inecolor238,13288
\definecolor {inecolor239,13345
\definecolor {inecolor240,13402
\definecolor {inecolor241,13459
\definecolor {inecolor242,13516
\definecolor {inecolor243,13573
\definecolor {inecolor244,13630
\definecolor {inecolor245,13687
\definecolor {inecolor246,13744
\definecolor {inecolor247,13801
\definecolor {inecolor248,13858
\definecolor {inecolor249,13915
\definecolor {inecolor250,13972
\definecolor {inecolor251,14029
\definecolor {inecolor252,14086
\definecolor {inecolor253,14143
\definecolor {inecolor254,14200
\definecolor {inecolor255,14257
\definecolor {inecolor256,14314
\definecolor {inecolor257,14371
\definecolor {inecolor258,14428
\definecolor {inecolor259,14485
\definecolor {inecolor260,14542
\definecolor {inecolor261,14599
\definecolor {inecolor262,14656
\definecolor {inecolor263,14713
\definecolor {inecolor264,14770
\definecolor {inecolor265,14827
\definecolor {inecolor266,14884
\definecolor {inecolor267,14941
\definecolor {inecolor268,14998
\definecolor {inecolor269,15055
\definecolor {inecolor270,15112
\definecolor {inecolor271,15169
\definecolor {inecolor272,15226
\definecolor {inecolor273,15283
\definecolor {inecolor274,15340
\definecolor {inecolor275,15397
\definecolor {inecolor276,15454
\definecolor {inecolor277,15511
\definecolor {inecolor278,15568
\definecolor {inecolor279,15625
\definecolor {inecolor280,15682
\definecolor {inecolor281,15739
\definecolor {inecolor282,15796
\definecolor {inecolor283,15853
\definecolor {inecolor284,15910
\definecolor {inecolor285,15967
\definecolor {inecolor286,16024
\definecolor {inecolor287,16081
\definecolor {inecolor288,16138
\definecolor {inecolor289,16195
\definecolor {inecolor290,16252
\definecolor {inecolor291,16309
\definecolor {inecolor292,16366
\definecolor {inecolor293,16423
\definecolor {inecolor294,16480
\definecolor {inecolor295,16537
\definecolor {inecolor296,16594
\definecolor {inecolor297,16651
\definecolor {inecolor298,16708
\definecolor {inecolor299,16765
\definecolor {inecolor300,16822
\definecolor {inecolor301,16879
\definecolor {inecolor302,16936
\definecolor {inecolor303,16993
\definecolor {inecolor304,17050
\definecolor {inecolor305,17107
\definecolor {inecolor306,17164
\definecolor {inecolor307,17221
\definecolor {inecolor308,17278
\definecolor {inecolor309,17335
\definecolor {inecolor310,17392
\definecolor {inecolor311,17449
\definecolor {inecolor312,17506
\definecolor {inecolor313,17563
\definecolor {inecolor314,17620
\definecolor {inecolor315,17677
\definecolor {inecolor316,17734
\definecolor {inecolor317,17791
\definecolor {inecolor318,17848
\definecolor {inecolor319,17905
\definecolor {inecolor320,17962
\definecolor {inecolor321,18019
\definecolor {inecolor322,18076
\definecolor {inecolor323,18133
\definecolor {inecolor324,18190
\definecolor {inecolor325,18247
\definecolor {inecolor326,18304
\definecolor {inecolor327,18361
\definecolor {inecolor328,18418
\definecolor {inecolor329,18475
\definecolor {inecolor330,18532
\definecolor {inecolor331,18589
\definecolor {inecolor332,18646
\definecolor {inecolor333,18703
\definecolor {inecolor334,18760
\definecolor {inecolor335,18817
\definecolor {inecolor336,18874
\definecolor {inecolor337,18931
\definecolor {inecolor338,18988
\definecolor {inecolor339,19045
\definecolor {inecolor340,19102
\definecolor {inecolor341,19159
\definecolor {inecolor342,19216
\definecolor {inecolor343,19273
\definecolor {inecolor344,19330
\definecolor {inecolor345,19387
\definecolor {inecolor346,19444
\definecolor {inecolor347,19501
\definecolor {inecolor348,19558
\definecolor {inecolor349,19615
\definecolor {inecolor350,19672
\definecolor {inecolor351,19729
\definecolor {inecolor352,19786
\definecolor {inecolor353,19843
\definecolor {inecolor354,19900
\definecolor {inecolor355,19957
\definecolor {inecolor356,20014
\definecolor {inecolor357,20071
\definecolor {inecolor358,20128
\definecolor {inecolor359,20185
\definecolor {inecolor360,20242
\definecolor {inecolor361,20299
\definecolor {inecolor362,20356
\definecolor {inecolor363,20413
\definecolor {inecolor364,20470
\definecolor {inecolor365,20527
\definecolor {inecolor366,20584
\definecolor {inecolor367,20641
\definecolor {inecolor368,20698
\definecolor {inecolor369,20755
\definecolor {inecolor370,20812
\definecolor {inecolor371,20869
\definecolor {inecolor372,20926
\definecolor {inecolor373,20983
\definecolor {inecolor374,21040
\definecolor {inecolor375,21097
\definecolor {inecolor376,21154
\definecolor {inecolor377,21211
\definecolor {inecolor378,21268
\definecolor {inecolor379,21325
\definecolor {inecolor380,21382
\definecolor {inecolor381,21439
\definecolor {inecolor382,21496
\definecolor {inecolor383,21553
\definecolor {inecolor384,21610
\definecolor {inecolor385,21667
\definecolor {inecolor386,21724
\definecolor {inecolor387,21781
\definecolor {inecolor388,21838
\definecolor {inecolor389,21895
\definecolor {inecolor390,21952
\definecolor {inecolor391,22009
\definecolor {inecolor392,22066
\definecolor {inecolor393,22123
\definecolor {inecolor394,22180
\definecolor {inecolor395,22237
\definecolor {inecolor396,22294
\definecolor {inecolor397,22351
\definecolor {inecolor398,22408
\definecolor {inecolor399,22465
\definecolor {inecolor400,22522
\definecolor {inecolor401,22579
\definecolor {inecolor402,22636
\definecolor {inecolor403,22693
\definecolor {inecolor404,22750
\definecolor {inecolor405,22807
\definecolor {inecolor406,22864
\definecolor {inecolor407,22921
\definecolor {inecolor408,22978
\definecolor {inecolor409,23035
\definecolor {inecolor410,23092
\definecolor {inecolor411,23149
\definecolor {inecolor412,23206
\definecolor {inecolor413,23263
\definecolor {inecolor414,23320
\definecolor {inecolor415,23377
\definecolor {inecolor416,23434
\definecolor {inecolor417,23491
\definecolor {inecolor418,23548
\definecolor {inecolor419,23605
\definecolor {inecolor420,23662
\definecolor {inecolor421,23719
\definecolor {inecolor422,23776
\definecolor {inecolor423,23833
\definecolor {inecolor424,23890
\definecolor {inecolor425,23947
\definecolor {inecolor426,24004
\definecolor {inecolor427,24061
\definecolor {inecolor428,24118
\definecolor {inecolor429,24175
\definecolor {inecolor430,24232
\definecolor {inecolor431,24289
\definecolor {inecolor432,24346
\definecolor {inecolor433,24403
\definecolor {inecolor434,24460
\definecolor {inecolor435,24517
\definecolor {inecolor436,24574
\definecolor {inecolor437,24631
\definecolor {inecolor438,24688
\definecolor {inecolor439,24745
\definecolor {inecolor440,24802
\definecolor {inecolor441,24859
\definecolor {inecolor442,24916
\definecolor {inecolor443,24973
\definecolor {inecolor444,25030
\definecolor {inecolor445,25087
\definecolor {inecolor446,25144
\definecolor {inecolor447,25201
\definecolor {inecolor448,25258
\definecolor {inecolor449,25315
\definecolor {inecolor450,25372
\definecolor {inecolor451,25429
\definecolor {inecolor452,25486
\definecolor {inecolor453,25543
\definecolor {inecolor454,25600
\definecolor {inecolor455,25657
\definecolor {inecolor456,25714
\definecolor {inecolor457,25771
\definecolor {inecolor458,25828
\definecolor {inecolor459,25885
\definecolor {inecolor460,25942
\definecolor {inecolor461,25999
\definecolor {inecolor462,26056
\definecolor {inecolor463,26113
\definecolor {inecolor464,26170
\definecolor {inecolor465,26227
\definecolor {inecolor466,26284
\definecolor {inecolor467,26341
\definecolor {inecolor468,26398
\definecolor {inecolor469,26455
\definecolor {inecolor470,26512
\definecolor {inecolor471,26569
\definecolor {inecolor472,26626
\definecolor {inecolor473,26683
\definecolor {inecolor474,26740
\definecolor {inecolor475,26797
\definecolor {inecolor476,26854
\definecolor {inecolor477,26911
\definecolor {inecolor478,26968
\definecolor {inecolor479,27025
\definecolor {inecolor480,27082
\definecolor {inecolor481,27139
\definecolor {inecolor482,27196
\definecolor {inecolor483,27253
\definecolor {inecolor484,27310
\definecolor {inecolor485,27367
\definecolor {inecolor486,27424
\definecolor {inecolor487,27481
\definecolor {inecolor488,27538
\definecolor {inecolor489,27595
\definecolor {inecolor490,27652
\definecolor {inecolor491,27709
\definecolor {inecolor492,27766
\definecolor {inecolor493,27823
\definecolor {inecolor494,27880
\definecolor {inecolor495,27937
\definecolor {inecolor496,27994
\definecolor {inecolor497,28051
\definecolor {inecolor498,28108
\definecolor {inecolor499,28165
\definecolor {inecolor500,28222
\definecolor {inecolor501,28279
\definecolor {inecolor502,28336
\definecolor {inecolor503,28393
\definecolor {inecolor504,28450
\definecolor {inecolor505,28507
\definecolor {inecolor506,28564
\definecolor {inecolor507,28621
\definecolor {inecolor508,28678
\definecolor {inecolor509,28735
\definecolor {inecolor510,28792
\definecolor {inecolor511,28849
\definecolor {inecolor512,28906
\definecolor {inecolor513,28963
\definecolor {inecolor514,29020
\definecolor {inecolor515,29077
\definecolor {inecolor516,29134
\definecolor {inecolor517,29191
\definecolor {inecolor518,29248
\definecolor {inecolor519,29305

rs_macros_colors.tex,565
\newcommand{\blue}\blue11,427
\newcommand{\darkblue}\darkblue12,471
\newcommand{\lightblue}\lightblue13,519
\newcommand{\red}\red14,574
\newcommand{\green}\green15,616
\newcommand{\lightgreen}\lightgreen16,666
\newcommand{\violet}\violet17,722
\newcommand{\darkviolet}\darkviolet18,770
\newcommand{\darkgrey}\darkgrey19,826
\newcommand{\palegrey}\palegrey20,878
\newcommand{\gray}\gray21,931
\newcommand{\white}\white22,975
\newcommand{\black}\black23,1021
\newcommand{\orange}\orange24,1067
\newcommand{\darkorange}\darkorange25,1115

rs_macros_dl.tex,2455
\newcommand{\en}\en7,256
\newcommand{\den}\den8,287
\newcommand{\mc}\mc10,334
\newcommand{\msf}\msf11,381
\newcommand{\snomed}\snomed13,429
\newcommand{\geneonto}\geneonto14,477
\newcommand{\nci}\nci15,530
\newcommand{\galen}\galen16,569
\newcommand{\shsnomed}\shsnomed18,613
\newcommand{\shnci}\shnci19,663
\newcommand{\shgalen}\shgalen20,705
\newcommand{\shfullgalen}\shfullgalen21,753
\newcommand{\shgeneontology}\shgeneontology22,808
\newcommand{\conj}\conj24,866
\newcommand{\disj}\disj25,893
\newcommand{\exr}\exr26,920
\newcommand{\subs}\subs28,958
\newcommand{\sups}\sups29,990
\newcommand{\norm}\norm30,1022
\newcommand{\comp}\comp31,1053
\newcommand{\topt}\topt33,1080
\newcommand{\bott}\bott34,1125
\newcommand{\conjt}\conjt35,1170
\newcommand{\disjt}\disjt36,1227
\newcommand{\exrt}\exrt37,1284
\newcommand{\equivt}\equivt38,1342
\newcommand{\subst}\subst39,1400
\newcommand{\supst}\supst40,1462
\newcommand{\pr}\pr44,1639
\newcommand{\prc}\prc45,1687
\newcommand{\sel}\sel46,1738
\newcommand{\selc}\selc47,1787
\newcommand{\goal}\goal49,1840
\newcommand{\goalsure}\goalsure50,1896
\newcommand{\tgoal}\tgoal51,1957
\newcommand{\igoal}\igoal52,2019
\newcommand{\sgoal}\sgoal53,2088
\newcommand{\isgoal}\isgoal54,2142
\newcommand{\nsgoal}\nsgoal55,2205
\newcommand{\assumptiongoal}\assumptiongoal57,2275
\newcommand{\assumptionsgoal}\assumptionsgoal58,2353
\newcommand{\aenc}\aenc60,2420
\newcommand{\wffsubs}\wffsubs61,2476
\newcommand{\wffsubsnotrans}\wffsubsnotrans62,2531
\newcommand{\wffmina}\wffmina63,2603
\newcommand{\wffminarule}\wffminarule64,2661
\newcommand{\wffminaT}\wffminaT65,2728
\newcommand{\wffminaTrule}\wffminaTrule66,2791
\newcommand{\wffallmina}\wffallmina67,2858
\newcommand{\wffallminarule}\wffallminarule68,2919
\newcommand{\wffallminaT}\wffallminaT69,2991
\newcommand{\wffallminaTrule}\wffallminaTrule70,3057
\newcommand{\wffallminaO}\wffallminaO71,3132
\newcommand{\wffallminaruleO}\wffallminaruleO72,3197
\newcommand{\pinpointingwff}\pinpointingwff74,3271
\newcommand{\pinpointingwffall}\pinpointingwffall75,3334
\newcommand{\hatT}\hatT77,3399
\newcommand{\Tp}\Tp78,3448
\newcommand{\elsat}\elsat80,3513
\newcommand{\el}\el96,3577
\newcommand{\elh}\elh97,3628
\newcommand{\elp}\elp98,3681
\newcommand{\elpp}\elpp99,3737
\newcommand{\eloh}\eloh100,3795
\newcommand{\eqdef}\eqdef101,3850

rs_macros_general.tex,3641
\newcommand{\RSHIGHLIGHT}\RSHIGHLIGHT19,616
\newcommand{\new}\new24,760
\newcommand{\ex}\ex25,795
\newcommand{\resp}\resp28,860
\newcommand{\done}\done29,894
\newcommand{\TODO}\TODO33,1016
\newcommand{\ACTODO}\ACTODO34,1042
\newcommand{\RS}\RS35,1111
\newcommand{\ignore}\ignore36,1153
\newcommand{\todo}\todo38,1256
\newcommand{\RSCHANGE}\RSCHANGE39,1281
\renewcommand{\RS}\RS40,1334
\newcommand{\PT}\PT41,1383
\newcommand{\RSTODO}\RSTODO42,1431
\renewcommand{\RSTODO}\RSTODO43,1506
\newcommand{\nota}\nota45,1567
\newcommand{\marg}\marg46,1624
\renewcommand{\marg}\marg47,1674
\newenvironment{rschange}rschange49,1747
\newenvironment{rs}rs50,1806
\newenvironment{pt}pt51,1859
\newcommand{\RSNOTE}\RSNOTE53,1914
\renewcommand{\RSNOTE}\RSNOTE55,2013
 \newcommand{\ignoreinshort}\ignoreinshort58,2101
 \newcommand{\ignoreinlong}\ignoreinlong59,2135
\def\makenewenumerate#1#2{\makenewenumerate67,2438
\newenvironment{#1}%69,2485
 \setlength{\labelwidth}width74,2633
\def\newplaintheorem#1#2{\newplaintheorem88,3171
\newenvironment{#1}{\begin{#1plain}\rm }{\end{#1plain}}}90,3233
\newcommand{\fakesubsubsection}\fakesubsubsection109,3990
\newcommand{\sref}\sref115,4148
\newcommand{\noi}\noi116,4184
\newcommand{\pair}\pair122,4311
\newcommand{\triple}\triple123,4378
\newcommand{\tuple}\tuple124,4452
\newcommand{\set}\set125,4515
\newcommand{\imp}\imp126,4566
\newcommand{\limp}\limp127,4617
\renewcommand{\iff}\iff128,4668
\newcommand{\defas}\defas129,4725
\newcommand{\thus}\thus130,4797
\newcommand{\pos}\pos132,4854
\newcommand\cala{\cala140,5006
\newcommand\calb{\calb141,5056
\newcommand\calc{\calc142,5106
\newcommand\cald{\cald143,5156
\newcommand\cale{\cale144,5206
\newcommand\calf{\calf145,5256
\newcommand\calg{\calg146,5306
\newcommand\calh{\calh147,5356
\newcommand\cali{\cali148,5406
\newcommand\calj{\calj149,5456
\newcommand\calk{\calk150,5506
\newcommand\call{\call151,5556
\newcommand\calm{\calm152,5606
\newcommand\caln{\caln153,5656
\newcommand\calo{\calo154,5706
\newcommand\calp{\calp155,5756
\newcommand\calq{\calq156,5806
\newcommand\calr{\calr157,5856
\newcommand\cals{\cals158,5906
\newcommand\calt{\calt159,5956
\newcommand\calu{\calu160,6006
\newcommand\calv{\calv161,6056
\newcommand\calw{\calw162,6106
\newcommand\calx{\calx163,6156
\newcommand\caly{\caly164,6206
\newcommand\calz{\calz165,6256
\newcommand{\rone}\rone172,6485
\newcommand{\rtwo}\rtwo173,6550
\newcommand{\rthree}\rthree174,6615
\newcommand{\ronetwo}\ronetwo175,6682
\newcommand{\ronethree}\ronethree176,6762
\newcommand{\ronefour}\ronefour178,6845
\newcommand{\rtwothree}\rtwothree179,6926
\newcommand{\rtwofour}\rtwofour180,7008
\newcommand{\ronetwothree}\ronetwothree182,7090
\newcommand{\ronethreefour}\ronethreefour184,7186
\newcommand{\rtwothreefour}\rtwothreefour186,7283
\newcommand{\ronetwothreefour}\ronetwothreefour189,7382
\renewcommand{\RSCHANGE}\RSCHANGE193,7497
\newcommand{\RSCHANGEONE}\RSCHANGEONE195,7587
\newcommand{\RSCHANGETWO}\RSCHANGETWO196,7648
\newcommand{\RSCHANGETHREE}\RSCHANGETHREE197,7709
\newcommand{\RSCHANGEONETHREE}\RSCHANGEONETHREE198,7774
\newcommand{\RSCHANGEONETWO}\RSCHANGEONETWO199,7845
\newcommand{\RSCHANGETWOTHREE}\RSCHANGETWOTHREE200,7912
\newcommand{\RSCHANGEFOUR}\RSCHANGEFOUR202,7984
\newcommand{\RSCHANGEONEFOUR}\RSCHANGEONEFOUR203,8047
\newcommand{\RSCHANGETWOFOUR}\RSCHANGETWOFOUR204,8116
\newcommand{\RSCHANGETHREEFOUR}\RSCHANGETHREEFOUR205,8185
\newcommand{\RSCHANGEONETHREEFOUR}\RSCHANGEONETHREEFOUR206,8261

rs_macros_mc.tex,1492
\newcommand{\nusmv}\nusmv7,256
\newcommand{\PROMELA}\PROMELA8,289
\newcommand{\smv}\smv9,326
\newcommand{\bdds}\bdds11,356
\newcommand{\bdd}\bdd12,395
\newcommand{\dis}\dis14,466
\newcommand{\con}\con15,490
\newcommand{\liff}\liff16,516
\newcommand{\true}\true17,552
\newcommand{\false}\false18,577
\newcommand{\CTL}\CTL19,603
\newcommand{\LTL}\LTL20,642
\newcommand{\E}\E26,700
\newcommand{\A}\A27,727
\newcommand{\G}\G28,754
\newcommand{\F}\F29,781
\newcommand{\U}\U30,808
\newcommand{\R}\R31,835
\newcommand{\X}\X32,862
\newcommand{\AG}\AG33,889
\newcommand{\AF}\AF34,918
\newcommand{\AU}\AU35,947
\newcommand{\AR}\AR36,976
\newcommand{\AX}\AX37,1005
\newcommand{\EG}\EG38,1034
\newcommand{\EF}\EF39,1063
\newcommand{\EU}\EU40,1092
\newcommand{\ER}\ER41,1121
\newcommand{\EX}\EX42,1150
\newcommand{\n}\n44,1180
\newcommand{\kil}\kil45,1212
\newcommand{\ki}\ki46,1257
\renewcommand{\k}\k47,1293
\newcommand{\kl}\kl48,1328
\newcommand{\fkil}\fkil50,1365
\newcommand{\fki}\fki51,1404
\newcommand{\fk}\fk52,1440
\newcommand{\fkl}\fkl53,1470
\newcommand{\gkil}\gkil55,1507
\newcommand{\gki}\gki56,1546
\newcommand{\gk}\gk57,1582
\newcommand{\gkl}\gkl58,1612
\newcommand{\Lkl}\Lkl60,1649
\newcommand{\Lkkll}\Lkkll61,1686
\newcommand{\Lkll}\Lkll62,1726
\newcommand{\Lk}\Lk63,1760
\newcommand{\Mkil}\Mkil65,1787
\newcommand{\Mki}\Mki66,1830
\newcommand{\Mk}\Mk67,1870
\newcommand{\Mkl}\Mkl68,1907

rs_macros_optsmt.tex,7331
\newcommand{\omtproblem}\omtproblem17,462
\newcommand{\omt}\omt18,526
\newcommand{\bomt}\bomt19,576
\newcommand{\omtt}\omtt20,628
\newcommand{\bomtt}\bomtt21,685
\newcommand{\omtplus}\omtplus23,745
\newcommand{\omlarat}\omlarat24,808
\newcommand{\omlaint}\omlaint25,870
\newcommand{\omla}\omla26,932
\newcommand{\omlaintplus}\omlaintplus27,988
\newcommand{\omlaratplus}\omlaratplus28,1060
\newcommand{\omlaplus}\omlaplus29,1132
\newcommand{\smtlaratplus}\smtlaratplus31,1199
\newcommand{\laratplus}\laratplus32,1255
\newcommand{\costfs}\costfs36,1338
\newcommand{\costfgen}\costfgen37,1398
\newcommand{\costfi}\costfi38,1457
\newcommand{\costfone}\costfone39,1492
\newcommand{\costfM}\costfM40,1529
\newcommand{\costs}\costs43,1588
\newcommand{\costgen}\costgen44,1643
\newcommand{\costi}\costi45,1698
\newcommand{\costone}\costone46,1731
\newcommand{\costM}\costM47,1766
\newcommand{\vvgen}\vvgen50,1824
\newcommand{\vvi}\vvi51,1886
\newcommand{\wvgen}\wvgen52,1922
\newcommand{\wvi}\wvi53,1984
\newcommand{\xvgen}\xvgen54,2020
\newcommand{\xvi}\xvi55,2082
\newcommand{\yvgen}\yvgen56,2118
\newcommand{\yvi}\yvi57,2180
\newcommand{\lbgen}\lbgen61,2234
\newcommand{\ubgen}\ubgen62,2297
\newcommand{\lb}\lb63,2360
\newcommand{\ub}\ub64,2389
\newcommand{\lbi}\lbi65,2418
\newcommand{\ubi}\ubi66,2449
\newcommand{\lbone}\lbone67,2480
\newcommand{\ubone}\ubone68,2513
\newcommand{\lbM}\lbM69,2546
\newcommand{\ubM}\ubM70,2577
\newcommand{\lbigen}\lbigen71,2608
\newcommand{\ubigen}\ubigen72,2649
\newcommand{\lbimax}\lbimax73,2690
\newcommand{\ubimin}\ubimin74,2727
\newcommand{\lbonemax}\lbonemax75,2764
\newcommand{\ubonemin}\ubonemin76,2803
\newcommand{\pivot}\pivot78,2843
\newcommand{\trueval}\trueval79,2899
\newcommand{\falseval}\falseval80,2951
\newcommand{\tpredgen}\tpredgen82,3020
\newcommand{\tpredigen}\tpredigen83,3084
\newcommand{\tpredij}\tpredij84,3129
\newcommand{\predgen}\predgen85,3166
\newcommand{\predigen}\predigen86,3226
\newcommand{\predij}\predij87,3269
\newcommand{\predonej}\predonej88,3304
\newcommand{\Agen}\Agen91,3413
\newcommand{\Aj}\Aj92,3463
\newcommand{\aij}\aij93,3490
\newcommand{\bi}\bi94,3542
\newcommand{\cj}\cj95,3592
\newcommand{\ddj}\ddj96,3642
\newcommand{\lj}\lj97,3693
\newcommand{\cgen}\cgen100,3761
\newcommand{\cigen}\cigen101,3826
\newcommand{\cijgen}\cijgen102,3891
\newcommand{\cijone}\cijone103,3956
\newcommand{\cijtwo}\cijtwo104,4017
\newcommand{\cij}\cij105,4078
\newcommand{\conej}\conej106,4135
\newcommand{\cc}\cc108,4195
\newcommand{\bounds}\bounds111,4245
\newcommand{\boundi}\boundi112,4310
\newcommand{\icost}\icost114,4377
\newcommand{\icostgen}\icostgen115,4427
\newcommand{\icosti}\icosti117,4560
\newcommand{\icostij}\icostij118,4626
\newcommand{\icostonej}\icostonej119,4681
\newcommand{\bcost}\bcost121,4748
\newcommand{\cost}\cost122,4798
\renewcommand{\costs}\costs123,4845
\newcommand{\mincost}\mincost124,4896
\newcommand{\bound}\bound125,4949
\newcommand{\guess}\guess126,4998
\newcommand{\oldguess}\oldguess127,5047
\newcommand{\oldbound}\oldbound128,5102
\newcommand{\maxboundi}\maxboundi129,5157
\newcommand{\maxboundone}\maxboundone130,5224
\newcommand{\nextsmallerbound}\nextsmallerbound131,5293
\newcommand{\noroom}\noroom132,5364
\newcommand{\mustbe}\mustbe133,5415
\newcommand{\bleft}\bleft134,5466
\newcommand{\bright}\bright135,5515
\newcommand{\pending}\pending136,5565
\newcommand{\tite}\tite138,5623
\newcommand{\ite}\ite139,5669
\newcommand{\costof}\costof141,5715
\newcommand{\costiof}\costiof142,5782
\newcommand{\mcostof}\mcostof143,5823
\newcommand{\mcostiof}\mcostiof144,5892
\newcommand{\C}\C148,5957
\newcommand{\Clemma}\Clemma149,6006
\newcommand{\Csolver}\Csolver150,6044
\newcommand{\incsmttc}\incsmttc156,6217
\newcommand{\smttcost}\smttcost157,6289
\newcommand{\smttc}\smttc158,6353
\newcommand{\smtc}\smtc159,6412
\newcommand{\Tlaint}\Tlaint160,6469
\newcommand{\smttlaint}\smttlaint161,6524
\newcommand{\optsmttc}\optsmttc164,6596
\newcommand{\decproblem}\decproblem166,6661
\newcommand{\optproblem}\optproblem167,6735
\newcommand{\vic}\vic170,6813
\newcommand{\eqij}\eqij173,6887
\newcommand{\neqij}\neqij174,6937
\newcommand{\dij}\dij175,6992
\newcommand{\dji}\dji176,7041
\newcommand{\muc}\muc180,7108
\newcommand{\mucgen}\mucgen181,7156
\newcommand{\muci}\muci182,7215
\newcommand{\mut}\mut183,7246
\newcommand{\mub}\mub184,7294
\newcommand{\mularat}\mularat186,7346
\newcommand{\mubool}\mubool187,7402
\newcommand{\mue}\mue189,7462
\newcommand{\mud}\mud190,7509
\newcommand{\mui}\mui191,7556
\newcommand{\mued}\mued192,7603
\newcommand{\muei}\muei193,7652
\newcommand{\mueid}\mueid194,7701
\newcommand{\murelaxed}\murelaxed196,7753
\newcommand{\Jplus}\Jplus202,7827
\newcommand{\Jminus}\Jminus203,7875
\newcommand{\Kplus}\Kplus204,7924
\newcommand{\Kminus}\Kminus205,7972
\newcommand{\Kplusone}\Kplusone206,8021
\newcommand{\Kminusone}\Kminusone207,8072
\newcommand{\Ilaint}\Ilaint211,8146
\newcommand{\IT}\IT212,8203
\newcommand{\I}\I213,8252
\newcommand{\mathsatC}\mathsatC216,8315
\newcommand{\scip}\scip217,8348
\newcommand{\bsolo}\bsolo218,8386
\newcommand{\satforj}\satforj219,8426
\newcommand{\pbclasp}\pbclasp220,8468
\newcommand{\bl}\bl223,8525
\newcommand\mysout{\mysout229,8646
\newcommand\nosout{\nosout230,8698
\definecolor{inecolor231,8750
\definecolor{inecolor232,8792
\def \gbox #1{\gbox233,8835
\newcommand{\fal}\fal234,8874
\newcommand{\tru}\tru235,8926
\newcommand{\mycite}\mycite237,8959
\newcommand{\mcite}\mcite238,9027
\newcommand{\mueuf}\mueuf241,9124
\newcommand{\mulaint}\mulaint242,9176
\newcommand{\infrule}\infrule243,9232
\newcommand{\hyp}\hyp244,9298
\newcommand{\comb}\comb245,9337
\newcommand{\fakeinfrule}\fakeinfrule247,9379
\newcommand{\currlb}\currlb252,9508
\newcommand{\currub}\currub253,9561
\newcommand{\range}\range254,9614
\newcommand{\currrange}\currrange255,9665
\newcommand{\lpivotrange}\lpivotrange256,9728
\newcommand{\rpivotrange}\rpivotrange257,9792
\newcommand{\computepivot}\computepivot258,9856
\newcommand{\dopivoting}\dopivoting260,9989
\newcommand{\ubliti}\ubliti262,10058
\newcommand{\lbliti}\lbliti263,10116
\newcommand{\pivotatom}\pivotatom264,10178
\newcommand{\currlblit}\currlblit265,10236
\newcommand{\currublit}\currublit266,10303
\newcommand{\currubliti}\currubliti267,10366
\newcommand{\negcurrubliti}\negcurrubliti268,10438
\newcommand{\minvalue}\minvalue270,10518
\newcommand{\maxvalue}\maxvalue271,10575
\newcommand{\mvalue}\mvalue272,10632
\renewcommand{\mincost}\mincost273,10685
\newcommand{\minimize}\minimize275,10750
\newcommand{\isminimum}\isminimum276,10812
\newcommand{\incrementalsmt}\incrementalsmt278,10951
\newcommand{\smtcoreextract}\smtcoreextract279,11031
\newcommand{\incrementalsmtcore}\incrementalsmtcore280,11111
\newcommand{\laqliterals}\laqliterals281,11208
\newcommand{\optimathsat}\optimathsat284,11284
\newcommand{\optmathsat}\optmathsat285,11339
\newcommand{\symba}\symba286,11393
\newcommand{\nuz}\nuz287,11436
\newcommand{\bclt}\bclt288,11479

rs_macros_sat.tex,1261
\newcommand{\dpll}\dpll13,424
\newcommand{\zchaff}\zchaff17,541
\newcommand{\satelite}\satelite18,590
\newcommand{\siege}\siege19,642
\newcommand{\berkmin}\berkmin20,690
\newcommand{\minisat}\minisat21,740
\newcommand{\minisattwo}\minisattwo22,790
\newcommand{\pickassign}\pickassign28,924
\newcommand{\picknewassign}\picknewassign29,992
\newcommand{\picktotalassign}\picktotalassign30,1075
\newcommand{\decidebranch}\decidebranch31,1151
\newcommand{\decide}\decide32,1224
\newcommand{\blevel}\blevel33,1278
\newcommand{\analyzeconflict}\analyzeconflict34,1332
\newcommand{\analyzededuction}\analyzededuction35,1406
\newcommand{\backtrack}\backtrack36,1482
\newcommand{\bcp}\bcp37,1542
\newcommand{\satres}\satres40,1637
\newcommand{\unsatres}\unsatres41,1679
\newcommand{\unknownres}\unknownres42,1725
\newcommand{\conflres}\conflres43,1775
\newcommand{\walksat}\walksat46,1858
\newcommand{\basicwalksmt}\basicwalksmt47,1896
\newcommand{\walksmt}\walksmt48,1954
\newcommand{\tpreprocess}\tpreprocess50,2002
\newcommand{\initialtruthassignment}\initialtruthassignment51,2058
\newcommand{\chooseunsatisfiedclause}\chooseunsatisfiedclause52,2132
\newcommand{\nexttruthassignment}\nexttruthassignment53,2208

rs_macros_smt.tex,5763
\newcommand{\proptofol}\proptofol16,473
\newcommand{\foltoprop}\foltoprop17,536
\newcommand{\btot}\btot18,599
\newcommand{\ttob}\ttob19,630
\newcommand{\vi}\vi27,934
\newcommand{\vip}\vip28,980
\newcommand{\mup}\mup29,1029
\newcommand{\muone}\muone30,1074
\newcommand{\mutwo}\mutwo31,1121
\newcommand{\muonetwo}\muonetwo32,1168
\newcommand{\taup}\taup33,1229
\newcommand{\etap}\etap34,1276
\newcommand{\cp}\cp35,1323
\newcommand{\atoms}\atoms37,1366
\newcommand{\B}\B42,1496
\newcommand{\T}\T43,1545
\newcommand{\Tone}\Tone44,1594
\newcommand{\Ttwo}\Ttwo45,1639
\newcommand{\Tonetwo}\Tonetwo46,1684
\newcommand{\smt}\smt47,1743
\newcommand{\smtt}\smtt48,1773
\newcommand{\smttt}\smttt49,1828
\newcommand{\smttonettwo}\smttonettwo50,1887
\newcommand{\Ti}\Ti51,1955
\newcommand{\tmany}\tmany52,1998
\newcommand{\smtmany}\smtmany53,2054
\newcommand{\utvpi}\utvpi55,2127
\newcommand{\utvpiint}\utvpiint56,2184
\newcommand{\utvpirat}\utvpirat57,2256
\newcommand{\bool}\bool58,2328
\newcommand{\euf}\euf59,2383
\newcommand{\eq}\eq60,2436
\newcommand{\dl}\dl61,2486
\newcommand{\dlrat}\dlrat62,2537
\newcommand{\dlint}\dlint63,2603
\newcommand{\la}\la64,2669
\newcommand{\larat}\larat65,2720
\newcommand{\laint}\laint66,2786
\newcommand{\laratint}\laratint67,2852
\renewcommand{\la}\la69,2955
\renewcommand{\larat}\larat70,3008
\renewcommand{\laint}\laint71,3065
\renewcommand{\laratint}\laratint72,3122
\newcommand{\fl}\fl75,3183
\newcommand{\nla}\nla76,3234
\newcommand{\nlarat}\nlarat77,3287
\newcommand{\nlaint}\nlaint78,3355
\newcommand{\bv}\bv79,3423
\newcommand{\mem}\mem80,3474
\newcommand{\lists}\lists81,3526
\newcommand{\tonetwo}\tonetwo82,3580
\newcommand{\smteuf}\smteuf84,3637
\newcommand{\smtdl}\smtdl85,3672
\newcommand{\smtdlrat}\smtdlrat86,3705
\newcommand{\smtdlint}\smtdlint87,3744
\newcommand{\smtutvpi}\smtutvpi88,3783
\newcommand{\smtutvpirat}\smtutvpirat89,3822
\newcommand{\smtutvpiint}\smtutvpiint90,3867
\newcommand{\smtla}\smtla91,3912
\newcommand{\smtlarat}\smtlarat92,3945
\newcommand{\smtlaint}\smtlaint93,3984
\newcommand{\smtbv}\smtbv94,4023
\newcommand{\smtmem}\smtmem95,4056
\newcommand{\genmodels}\genmodels98,4093
\newcommand{\Tmodels}\Tmodels99,4134
\newcommand{\laratmodels}\laratmodels100,4170
\newcommand{\laintmodels}\laintmodels101,4214
\newcommand{\lamodels}\lamodels102,4258
\newcommand{\dlmodels}\dlmodels103,4296
\newcommand{\dlintmodels}\dlintmodels104,4334
\newcommand{\dlratmodels}\dlratmodels105,4378
\newcommand{\pmodels}\pmodels106,4422
\newcommand{\TsolverGen}\TsolverGen110,4531
\newcommand{\TsolversGen}\TsolversGen111,4601
\newcommand{\Tsolver}\Tsolver112,4673
\newcommand{\Tsolvers}\Tsolvers113,4712
\newcommand{\Psolver}\Psolver114,4753
\newcommand{\TTsolver}\TTsolver115,4803
\newcommand{\Tonesolver}\Tonesolver116,4859
\newcommand{\Ttwosolver}\Ttwosolver117,4917
\newcommand{\Tonetwosolver}\Tonetwosolver118,4975
\newcommand{\Tisolver}\Tisolver119,5046
\newcommand{\Tisolvers}\Tisolvers120,5100
\newcommand{\TdeduceGen}\TdeduceGen121,5156
\newcommand{\Tonededuce}\Tonededuce122,5226
\newcommand{\Ttwodeduce}\Ttwodeduce123,5284
\newcommand{\Tlemma}\Tlemma125,5343
\newcommand{\Tlemmas}\Tlemmas126,5381
\newcommand{\Tilemma}\Tilemma127,5421
\newcommand{\Tilemmas}\Tilemmas128,5461
\newcommand{\laratsolver}\laratsolver130,5504
\newcommand{\laratsolvers}\laratsolvers131,5567
\newcommand{\laintsolver}\laintsolver132,5632
\newcommand{\laintsolvers}\laintsolvers133,5695
\newcommand{\lasolver}\lasolver134,5760
\newcommand{\lasolvers}\lasolvers135,5817
\newcommand{\argolib}\argolib141,5954
\newcommand{\barcelogic}\barcelogic142,6001
\newcommand{\blast}\blast143,6054
\newcommand{\clp}\clp144,6097
\newcommand{\csisat}\csisat145,6143
\newcommand{\cvcthree}\cvcthree146,6188
\newcommand{\foci}\foci147,6233
\newcommand{\haRVey}\haRVey148,6274
\newcommand{\intjain}\intjain149,6319
\newcommand{\lifter}\lifter150,6363
\newcommand{\mathsat}\mathsat151,6408
\newcommand{\verifun}\verifun152,6455
\newcommand{\yices}\yices153,6503
\newcommand{\zapato}\zapato154,6546
\newcommand{\zap}\zap155,6593
\newcommand{\zthree}\zthree156,6632
\newcommand{\microformal}\microformal158,6674
\newcommand{\mathsatfour}\mathsatfour160,6730
\newcommand{\mathsatfive}\mathsatfive161,6782
\newcommand{\mathsatfivePrep}\mathsatfivePrep162,6834
\newcommand{\mathsatfiveCleaneling}\mathsatfiveCleaneling163,6917
\newcommand{\mathsatfiveMinisat}\mathsatfiveMinisat164,6995
\newcommand{\myeij}\myeij168,7152
\newcommand{\myeijs}\myeijs169,7200
\newcommand{\mynegeij}\mynegeij170,7250
\newcommand{\eij}\eij171,7306
\newcommand{\eik}\eik172,7353
\newcommand{\ejk}\ejk173,7400
\newcommand{\diseij}\diseij174,7447
\newcommand{\NO}\NO176,7501
\newcommand{\Bool}\Bool177,7560
\newcommand{\BoolGen}\BoolGen178,7614
\newcommand{\BoolT}\BoolT179,7679
\newcommand{\BoolTonetwo}\BoolTonetwo180,7712
\newcommand{\BoolTi}\BoolTi181,7757
\newcommand{\BoolNO}\BoolNO182,7795
\newcommand{\DelBoolNO}\DelBoolNO183,7831
\newcommand{\TsatisfiableGen}\TsatisfiableGen185,7913
\newcommand{\TsatGen}\TsatGen186,7993
\newcommand{\TunsatGen}\TunsatGen187,8057
\newcommand{\Tonesat}\Tonesat188,8125
\newcommand{\Ttwosat}\Ttwosat189,8175
\newcommand{\Toneunsat}\Toneunsat190,8225
\newcommand{\Ttwounsat}\Ttwounsat191,8279
\newcommand{\Tsatisfiable}\Tsatisfiable192,8333
\newcommand{\Psatisfiable}\Psatisfiable193,8381
\newcommand{\Tonesatisfiable}\Tonesatisfiable194,8441
\newcommand{\Ttwosatisfiable}\Ttwosatisfiable195,8507
\newcommand{\Tisatisfiable}\Tisatisfiable196,8573

rs_macros_specific.tex,1162
\renewcommand{\new}\new2,1
\renewcommand{\RSTODO}\RSTODO4,83
\renewcommand{\paragraph}\paragraph5,160
\newcommand{\alla}\alla8,223
\newcommand{\allb}\allb9,286
\renewcommand{\vi}\vi10,349
\newcommand{\vione}\vione11,407
\newcommand{\vitwo}\vitwo12,467
\renewcommand{\vi}\vi13,528
\renewcommand{\vione}\vione14,576
\renewcommand{\vitwo}\vitwo15,631
\newcommand{\ps}\ps16,686
\renewcommand{\trueval}\trueval18,746
\renewcommand{\falseval}\falseval19,789
\newcommand{\andmu}\andmu21,835
\newcommand{\andeta}\andeta22,891
\newcommand{\entails}\entails24,950
\newcommand{\validates}\validates25,981
\newcommand{\apply}\apply27,1014
\newcommand{\applymuvi}\applymuvi28,1067
\newcommand{\applyetavi}\applyetavi29,1116
\newcommand{\oksym}\oksym32,1169
\newcommand{\noksym}\noksym33,1253
\newcommand{\shannon}\shannon35,1338
\newcommand{\shannonpsib}\shannonpsib36,1400
\newcommand{\predabsphi}\predabsphi38,1450
\newcommand{\verbvalidate}\verbvalidate40,1525
\newcommand{\verbvalidates}\verbvalidates41,1562
\newcommand{\verbvalidating}\verbvalidating42,1601
\newcommand{\verbvalidation}\verbvalidation43,1642

statements.tex,604
\renewcommand{\topfraction}\topfraction6,108
\renewcommand{\bottomfraction}\bottomfraction7,139
\renewcommand{\textfraction}\textfraction8,173
\newcommand{\longversion}\longversion65,1559
  \renewcommand{\ignoreinshort}\ignoreinshort69,1637
  \renewcommand{\ignoreinshort}\ignoreinshort70,1694
  \renewcommand{\ignoreinlong}\ignoreinlong71,1735
 \renewcommand{\ignoreinshort}\ignoreinshort74,1777
 \renewcommand{\ignoreinlong}\ignoreinlong75,1813
\label{sec:}sec:128,2595
\section*{*142,3022
\section*{*208,4740
$\alla\defas\set{as\set212,4807
$\allb\defas\set{as\set213,4839

thanks.tex,48
\section{Acknowledgements}Acknowledgements1,0

todo.tex,17
\section*{*2,9

template_withfigure.tex,0

template.tex,0

template_2page.tex,0

concl.tex,0

abstract.tex,0


==> abstract.tex.1 <==
Many procedures for SAT and 
SAT-related problems --in particular those requiring the complete
enumeration of satisfying truth assignments--
rely their efficiency
on the detection of {\em partial} assignments satisfying an input
formula.
%
In this paper we analyze in deep the notion of partial-assignment
satisfiability. 
%
We start by raising a flag on the fact that by %ambiguity of the sentence 
``{\em a partial truth assignment $\mu$ satisfies a formula $\vi$}'',
we may  mean  either that $\mu$ {\em entails} $\vi$
(i.e. that all total assignments extending $\mu$
satisfy $\vi$) or that $\mu$ {\em validates} $\vi$ 
 (i.e. that applying $\mu$ to $\vi$ makes $\vi$ true).
%
% We start by raising a flag on the ambiguity of the sentence 
% ``{\em a partial truth assignment $\mu$ satisfies a formula $\vi$}'',
% which may  mean  either that $\mu$ {\em entails} $\vi$
% (i.e. ``all total assignments extending $\mu$
% satisfy $\vi$'') or that $\mu$ {\em validates} $\vi$ 
%  (i.e. ``applying $\mu$ to $\vi$ makes $\vi$ true'');
% %
We notice that, whereas for (tautology-free) CNF formulas entailment 
and validation are equivalent, for non-CNF formulas --and for
existentially-quantified formulas, even CNF ones--
{\em validation is strictly stronger than entailment}, and they have
complementary properties. 

\ignore{
Also, (Tseitin-style) CNF-ization does not solve this
issue, because 
%with Tseitin CNF-ization 
it may lose 
information regarding partial-assignment entailment or validation.
} 
The distinction between entailment and validation
%is not just an issue of terminology, rather it 
has important consequences at algorithmic level:
distinct algorithms implicitly use one or the other as 
satisfiablity criterium; checking entailment is much harder than
checking validation, but it allows for producing smaller partial
assignments, and hence possibly drastically reducing their number. 
This
 may drive the
development of more effective assignment-enumeration algorithms.
%


==> figure.tex <==
\newcommand{\mainwff}{\ensuremath{(A_1\wedge  A_2)\vee(A_1\wedge \neg A_2)}}
\newcommand{\wffl}{\ensuremath{(A_1\wedge  A_2)}}
\newcommand{\wffr}{\ensuremath{(A_1\wedge \neg A_2)}}
\newcommand{\Aone}{\ensuremath{A_1}}
\newcommand{\nAone}{\ensuremath{\neg A_1}}
\newcommand{\Atwo}{\ensuremath{A_2}}
\newcommand{\nAtwo}{\ensuremath{\neg A_2}}  
\newcommand{\singlemu}{\set{A_1}}
\newcommand{\allmus}{\set{\set{A_1,A_2},\set{A_1,\neg A_2}}}
% 
\begin{figure}[t]  
  \centering   
\scalebox{.8}{\input{comparison.pdf_t}} 
\caption{Left: OBDD for $\vi\defas\mainwff{}$. \newline
Center and right: Assignment enumeration for  $\vi$ via Analytic
Tableaux and (non-CNF) DPLL.
\label{fig:comparison}} 
\end{figure} 


==> intro_v1.tex <==
% Although  CDCL 
% \cite{MSLM09HBSAT} 
% and SLS \cite{Maj09HBSAT} SAT solvers return  {\em total} truth assignments
% satisfying the input formula, other SAT procedures 
Many procedures for for SAT and SAT-related problems
(e.g. OBDDs
\cite{bryant2}, Analytic Tableaux \cite{smullyan1}, DPLL
\cite{davis7}) rely their efficiency
on the detection of {\em partial} assignments satisfying an input
formula.
In particular,
when it comes to SAT-based problems requiring
the complete enumeration of satisfying assignments (e.g. \#SAT
\cite{GSS09HBSAT}, Lazy SMT \cite{BSST09HBSAT}, AllSAT and AllSMT
\cite{allsmt}, satisfiability of modal and description logics
\cite{ST09HBSAT}), the capability of enumerating  {\em
partial}  satisfying assignments which are as small as possible is often essential, because 
detecting that a partial assignment satisfies the input formula 
may avoid the enumeration of the whole subtree
of total assignments extending it, whose size is exponential in the
number of unassigned propositions.

% a satisfying partial
% assignment can be generated instead of the whole subtree
% of total assignments extending it, whose size is exponential in the
% number of unassigned propositions.

% When we deal with (tautology-free) CNF formulas, the notion of
% partial-assignment satisfiablity is clear SPIEGA E CITA. BOTH PROPERTIES

In this paper we analyze in deep the notion of partial-assignment
satisfiability. 
First we raise a flag on the fact that by
``{\em a partial truth assignment $\mu$ satisfies a formula $\vi$}'',
we may mean either that $\mu$ {\em entails} $\vi$
(i.e. that all total assignments extending $\mu$
satisfy $\vi$) or that $\mu$ {\em validates} $\vi$
 (i.e. that applying $\mu$ to $\vi$ makes $\vi$ true).
%
Typically most authors in the SAT community
leave this definition
implicit, or provide a definition only for (tautology-free) CNF
formulas (e.g. \cite{KBK09HBSAT}).
% where we notice that
% entailment and validation concide. 
%
We notice that, whereas for (tautology-free) CNF formulas entailment 
and validation are equivalent, for non-CNF formulas --and for
existentially-quantified formulas, even CNF ones--
{\em validation is strictly stronger than entailment}, and they have
complementary properties. 

We also notice that 
 (Tseitin-style) CNF-ization does not solve this
issue, because 
%with Tseitin CNF-ization 
it may lose 
information regarding partial-assignment entailment or validation.
%\ignoreinshort{\RSTODO{Mention Kripke \& C e Stefano Tonetta?}}
%We stress the fact that the 

We stress the fact that the distinction between entailment and validation
is not just an issue of terminology; rather, it 
has important consequences at
algorithmic level. 
%
We notice, e.g., that
OBDDs \cite{bryant2} implicitly enumerate partial assignment {\em entailing}
the input formulas, whereas Analytic Tableaux \cite{smullyan1} and
(non-CNF) DPLL \cite{davis7} implicitly enumerate partial assignment
{\em validating} it. 
%
Also, e.g., techniques like {\em pure-literal
filtering} 
%and {\em ghost-literal filtering} 
\cite{sebastiani07,BSST09HBSAT} in lazy
SMT 
implicitly aim at reducing a
total assignment to a partial one {\em validating} the input formula. 
%
On the one hand, checking entailment is computationally
much harder than checking
validation. On the other hand, since partial assignments entailing
$\vi$ are in general subsets of those validating $\vi$, being able
to produce  partial assignments
{\em entailing} the input formula rather than {\em validating} it
 allows for producing smaller partial assignments,
and hence possibly drastically reducing their number. 
This may drive the development of more effective assignment-enumeration algorithms.
%
% When it comes to enumerating, in order to maximizing efficiency
% we would like to produce  partial assignments
% entailing the input formula, although most 
% algorithms give us only partial assignments
% validating it.

%\RSTODO{Aggiungi riferimento a poll.\\}
\ignore{
\paragraph{A poll.}
In order to support the analysis, I've set up an email
poll among some current or past SAT PC and some SMT PC members, asking
for the truth/falsehood of five statements on the
notion of partial-assignment satisfiability.
The result are available at \cite{poll} %
%\footnote{\url{http://disi.unitn.it/rseba/partialsat_poll_2019.03.11.pdf}}
 and as an appendix submitted with this paper. 
Although only 20 out of 65 people replied, 
the result 
reveals the lack of general agreement among the repliers on the notion of
partial-assignment satisfiability and on its consequences: e.g.,
% since 
the repliers split evenly into supporters 
of entailment, of validation, and people considering them equivalent.
}


\paragraph{Personal note.} The analysis presented in this paper was
triggered
by the effort of conceiving more efficient procedures for predicate
abstraction in SMT for improving Weighted Model Integration
\cite{MorPasSeb17,morettin_aij19},
which forced me to elaborate on the distinction between entailment
and validation. Before then, I personally used to see
partial-assignment satisfiability as {entailment}
 (see \cite{gs-infocomp2000}) without paying attention to the distinction.

{\paragraph{Content.} The rest of the paper is organized as follows.
\sref{sec:background} provides the necessary notation, terminology
and concepts used in the paper.
\sref{sec:partialsat} introduces entailment and
validation for generic propositional formulas and discusses their
relative properties and use.
\sref{sec:partialsat-exist} lifts the discussion to
existentially-quantified formulas.
\sref{sec:concl} provides some conclusions and future-work suggestions.
}



==> intro_v2.tex <==
% Although  CDCL 
% \cite{MSLM09HBSAT} 
% and SLS \cite{Maj09HBSAT} SAT solvers return  {\em total} truth assignments
% satisfying the input formula, other SAT procedures 

\TODO{Cambiare la narrazione:
\\- we wish... however...
\\- Proporre da
qualche parte ``satisfy'' as ``entailment''.
\\- far notare come
tipicamente evaluation to true.
}

 \newpage
\marg{need for PAS}
Many procedures for SAT and SAT-related problems
(e.g. OBDDs
\cite{bryant2}, Analytic Tableaux \cite{smullyan1}, DPLL
\cite{davis7}) rely their efficiency
on the detection of {\em partial} truth assignments $\mu$  satisfying an input
 propositional formula $\vi$, which allows to
state that (i) $\vi$ is satisfiable and (ii) all total 
assignments extending $\mu$ satisfy \vi. 
% state not only that $\vi$ is satisfiable, but also that all total 
% assignments extending $\mu$ satisfy \vi. 
In particular,
when it comes to SAT-based problems requiring
the {\em complete enumeration} of satisfying assignments (e.g. \#SAT
\cite{GSS09HBSAT}, Lazy SMT \cite{BSST09HBSAT}, AllSAT and AllSMT
\cite{allsmt}, satisfiability of modal and description logics
\cite{ST09HBSAT}, Weighted Model Integration \cite{MorPasSeb17}),
%
the ability of enumerating satisfying {partial} assignments which are
as small as possible is essential, because
%detecting that a partial assignment satisfies the input formula 
each of them
avoids the enumeration of the whole subtree
of total assignments extending it, whose size is exponential in the
number of unassigned propositions.

\marg{no definition}
Surprisingly,
% despite its widespread (implicit) usage of
% partial-assignment satisfiablity
% in algorithms and
%apart from the case of (tautology-free) CNF formulas,
there seems to be no general and universally-agreed definition of
partial-assignment satisfaction:
most authors do not
define partial-assignment satisfaction explicitly, or define it only when dealing with
(tautology-free) CNF formulas (e.g.  \cite{KBK09HBSAT});
%
\marg{algos diff notions}
also, different algorithms implictly implement different notions of
partial-assignment satisfaction (see below).
%
% In order to be useful, such a definition should at least guarantee
% that, if a partial assignment $\mu$ satisfies a formula \vi, then (i)
% \vi is satisfiable and (ii) all total truth assignments extending it
% satisfy \vi.~%\footnote{

%\begin{remark}
We stress the fact that this is not simply an issue of
the meaning of the word ``satisfy'': whichever ``verb'' one
might  use for it (e.g. ``satisfy'', ``entail'', ``imply'', ``evaluate to
true'',...), we would like a universally-agreed criterion
to extablishing that, if a partial truth-assignment ``verbs'' a formula
$\vi$, then (i) $\vi$ is satisfiable and (ii) all total truth
 assignments extending it satisfy $\vi$. 
\ignore{
we need a universally-agreed criterion
 complying with the two conditions (i) and (ii)
above.
} 
%\end{remark}
%}
% a criterion the sentence
% ``a partial truth assignment $\mu$ [verb] a formula $\vi$'' should
% imply that (i) \vi is satisfiable and (ii) that all total truth
% assignments extending it satisfy \vi. 

% a satisfying partial
% assignment can be generated instead of the whole subtree
% of total assignments extending it, whose size is exponential in the
% number of unassigned propositions.

% When we deal with (tautology-free) CNF formulas, the notion of
% partial-assignment satisfiablity is clear SPIEGA E CITA. BOTH PROPERTIES

\ignore{In this paper 
analyze in deep the notion of partial-assignment
satisfiability,
raising  a flag about the ambiguities and subtleties
of this concept,
and highlighting their practical consequences.

In this paper we
raise  a flag about the ambiguities and subtleties
of partial-assignment
satisfiability, in particular for  non-CNF or
existentially-quantified formulas, 
and investigate their practical consequences.
}
%\TODO{We wish to fill this gap...}

\RSTODO{move up?}
In this paper we want to address this issue explicitly. We
analyze the notion of partial-assignment
satisfiability,
raising  a flag about the ambiguities and subtleties
of this concept  --in particular when dealing with  non-CNF and
existentially-quantified formulas-- 
and we investigate their practical consequences.

\marg{$\entails$ vs. $\validates$}
We start by noticing the following fact:
whereas for (tautology-free) CNF formulas
``{\em a partial truth assignment $\mu$ satisfies a formula $\vi$}''
may be indifferently be interpreted either as 
``$\mu$ {\em entails} $\vi$''
(i.e. ``all total assignments extending $\mu$
satisfy $\vi$'') or as ``$\mu$ {\em \verbvalidates{}} $\vi$''
 (i.e. ``applying $\mu$ to $\vi$ makes $\vi$ true'') because in this
 case the two  concepts are equivalent,
 %
 for non-CNF formulas instead --and for
existentially-quantified formulas, even CNF ones--
{\em \verbvalidation{} is strictly stronger than entailment}, and they have
complementary properties. 
%
\ignore{
First we raise a flag on the fact that by
``{\em a partial truth assignment $\mu$ satisfies a formula $\vi$}'',
we may mean either that $\mu$ {\em entails} $\vi$
(i.e. that all total assignments extending $\mu$
satisfy $\vi$) or that $\mu$ {\em \verbvalidates{}} $\vi$
 (i.e. that applying $\mu$ to $\vi$ makes $\vi$ true).
%
Typically most authors in the SAT community
leave this definition
implicit, or provide a definition only for (tautology-free) CNF
formulas (e.g. \cite{KBK09HBSAT}).
% where we notice that
% entailment and \verbvalidation{} concide. 
%
We notice that, whereas for (tautology-free) CNF formulas entailment 
and \verbvalidation{} are equivalent, for non-CNF formulas --and for
existentially-quantified formulas, even CNF ones--
{\em \verbvalidation{} is strictly stronger than entailment}, and they have
complementary properties. 
}
We also notice that standard
 (Tseitin-style) CNF-ization does not solve this
issue, because 
%with Tseitin CNF-ization 
it may lose 
information regarding partial-assignment entailment or \verbvalidation{}.
%\ignoreinshort{\TODO{Mention Kripke \& C e Stefano Tonetta?}}
%We stress the fact that the 

We also stress the fact that the distinction between entailment and \verbvalidation{}
is not only an issue of providing an universally-agreed definition of
partial-assignment satisfiability, but it also 
has important practical consequences. 
%
\RSTODO{Aggiungere $\validates$ vs. equivalence}
\RSTODO{Although...}
On the one hand, checking entailment is computationally
much harder than checking
\verbvalidation{}. On the other hand, since partial assignments entailing
$\vi$ are in general subsets of those \verbvalidating{} $\vi$, being able
to produce  partial assignments
{entailing} the input formula rather than {\verbvalidating{}} it
 allows for producing smaller partial assignments,
and hence possibly drastically reducing their number. 
This may drive the development of more effective assignment-enumeration algorithms.
%
% When it comes to enumerating, in order to maximizing efficiency
% we would like to produce  partial assignments
% entailing the input formula, although most 
% algorithms give us only partial assignments
% \verbvalidating{} it.

\marg{algos different notions of PAS}
To this extent we notice, e.g., that, when applied to non-CNF
formulas, 
OBDDs \cite{bryant2} implicitly enumerate partial assignment {entailing}
the input formulas,  whereas other procedures like Analytic Tableaux \cite{smullyan1} and
(non-CNF) DPLL \cite{davis7} implicitly enumerate partial assignment
{\verbvalidating{}} them. 
%
Also, e.g., techniques like {\em pure-literal
filtering} 
%and {\em ghost-literal filtering} 
\cite{sebastiani07,BSST09HBSAT} in lazy
SMT 
implicitly aim at reducing a
total assignment to a partial one {\verbvalidating{}} the input formula. 


%\TODO{Aggiungi riferimento a poll.\\}
\ignore{
\paragraph{A poll.}
In order to support the analysis, I've set up an email
poll among some current or past SAT PC and some SMT PC members, asking
for the truth/falsehood of five statements on the
notion of partial-assignment satisfiability.
The result are available at \cite{poll} %
%\footnote{\url{http://disi.unitn.it/rseba/partialsat_poll_2019.03.11.pdf}}
 and as an appendix submitted with this paper. 
Although only 20 out of 65 people replied, 
the result 
reveals the lack of general agreement among the repliers on the notion of
partial-assignment satisfiability and on its consequences: e.g.,
% since 
the repliers split evenly into supporters 
of entailment, of \verbvalidation{}, and people considering them equivalent.
}


\paragraph{Motivation.} The analysis presented in this paper was
triggered
by the effort of conceiving more efficient procedures for predicate
abstraction in SMT for improving Weighted Model Integration
\cite{MorPasSeb17,morettin_aij19},
which forced me to elaborate on the distinction between entailment
and \verbvalidation{}. Before then, I personally used to see
partial-assignment satisfiability as {entailment}
 (see \cite{gs-infocomp2000}) without paying attention to the distinction.

{\paragraph{Content.} The rest of the paper is organized as follows.
\sref{sec:background} provides the necessary notation, terminology
and concepts used in the paper.
\sref{sec:partialsat} introduces entailment and
\verbvalidation{} for generic propositional formulas and discusses their
relative properties and use.
\sref{sec:partialsat-exist} lifts the discussion to
existentially-quantified formulas.
\sref{sec:concl} provides some conclusions and future-work suggestions.
}



==> todo.tex <==
\newpage
\section*{TODO}
\begin{itemize}
\item Everywhere
  \begin{itemize}
  \item 
  \item 
  \item
  \end{itemize}

\item INTRO
  \begin{itemize}
  \item add mention to poll
  \item add content
  \end{itemize}
\item background: 
  \begin{itemize}
  \item 
  \item 
  \end{itemize}
\item satisfiability
  \begin{itemize}
  \item 
  \item 
\item 
  \item 
  \end{itemize}
\item existential satisfiability
  \begin{itemize}
  \item 
  \item 
  \end{itemize}
\item POLL
  \begin{itemize}
  \item 
  \item 
  \end{itemize}
\end{itemize}



